DriveGazen: Event-Based Driving Status Recognition using Conventional Camera

We introduce a wearable driving status recognition device and our open-source dataset, along with a new real-time method robust to changes in lighting conditions for identifying driving status from eye observations of drivers. The core of our method is generating event frames from conventional intensity frames, and the other is a newly designed Attention Driving State Network (ADSN). Compared to event cameras, conventional cameras offer complete information and lower hardware costs, enabling captured frames to encode rich spatial information. However, these textures lack temporal information, posing challenges in effectively identifying driving status. DriveGazen addresses this issue from three perspectives. First, we utilize video frames to generate realistic synthetic dynamic vision sensor (DVS) events. Second, we adopt a spiking neural network to decode pertinent temporal information. Lastly, ADSN extracts crucial spatial cues from corresponding intensity frames and conveys spatial attention to convolutional spiking layers during both training and inference through a novel guide attention module to guide the feature learning and feature enhancement of the event frame. We specifically collected the Driving Status (DriveGaze) dataset to demonstrate the effectiveness of our approach. Additionally, we validate the superiority of the DriveGazen on the Single-eye Event-based Emotion (SEE) dataset. To the best of our knowledge, our method is the first to utilize guide attention spiking neural networks and eye-based event frames generated from conventional cameras for driving status recognition. Please refer to our project page for more details: https://github.com/TooyoungALEX/AAAI25-DriveGazen.

==> sections/checklist.tex <==
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage[submission]{aaai25}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet}  % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
% %
% % These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{upgreek}

% \usepackage{epsfig}
% \usepackage{amsmath}
% \usepackage{amssymb}

% % Include other packages here, before hyperref.
% \usepackage{array}
% \usepackage{diagbox}
% \usepackage{multirow}
% \usepackage{float}
% \usepackage{soul}
% \usepackage{ textcomp }
% \usepackage{paralist}
% \usepackage{soul}

% \usepackage{xcolor}

% \newcommand{\ylt}[1]{\textcolor[rgb]{0.0,0.0,0.0}{#1}}
% \newcommand{\red}[1]{\textcolor[rgb]{1,0,0}{#1}}
% \newcommand{\green}[1]{\textcolor[rgb]{0,1,0}{#1}}
% \newcommand{\blue}[1]{\textcolor[rgb]{0,0,1}{#1}}
% \newcommand{\ignorethis}[1]{}




% %
% % These are are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
% \usepackage{newfloat}
% \usepackage{listings}
% \DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
% \lstset{%
% 	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
% 	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
% 	aboveskip=0pt,belowskip=0pt,%
% 	showstringspaces=false,tabsize=2,breaklines=true}
% \floatstyle{ruled}
% \newfloat{listing}{tb}{lst}{}
% \floatname{listing}{Listing}
% %
% % Keep the \pdfinfo as shown here. There's no need
% % for you to add the /Title and /Author tags.
% \pdfinfo{
% /TemplateVersion (2025.1)
% }

% \setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.

% % Document starts
% \begin{document}
% % Title portion





\title{Checklist}

\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\red{yes}/partial/no/NA)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\red{yes}/no)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\red{yes}/no)
\end{itemize}




\noindent{Does this paper make theoretical contributions? (\red{yes}/no) }

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (\red{yes}/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (\red{yes}/partial/no)
    \item Proofs of all novel claims are included. (\red{yes}/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (\red{yes}/partial/no)
    \item Appropriate citations to theoretical tools used are given. (\red{yes}/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (\red{yes}/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (\red{yes}/no/NA)
\end{itemize}





\noindent{Does this paper rely on one or more datasets? (\red{yes}/no) }

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\red{yes}/partial/no/NA)
    \item All novel datasets introduced in this paper are included in a data appendix. (\red{yes}/partial/no/NA)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\red{yes}/partial/no/NA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\red{yes}/no/NA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\red{yes}/partial/no/NA)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\red{yes}/partial/no/NA)
\end{itemize}




\noindent{Does this paper include computational experiments? (\red{yes}/no) }

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (\red{yes}/partial/no).
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\red{yes}/partial/no)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\red{yes}/partial/no)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\red{yes}/partial/no)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\red{yes}/partial/no/NA)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\red{yes}/partial/no)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\red{yes}/partial/no)
    \item This paper states the number of algorithm runs used to compute each reported result. (\red{yes}/no)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\red{yes}/no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\red{yes}/partial/no)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\red{yes}/partial/no/NA)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\red{yes}/partial/no/NA)
\end{itemize}






% \end{document}
